Artificial Intelligence in Dry Eye Disease

Dry eye disease (DED) has a prevalence of between 5 and 50\%, depending on the diagnostic criteria used and population under study. However, it remains one of the most underdiagnosed and undertreated conditions in ophthalmology. Many tests used in the diagnosis of DED rely on an experienced observer for image interpretation, which may be considered subjective and result in variation in diagnosis. Since artificial intelligence (AI) systems are capable of advanced problem solving, use of such techniques could lead to more objective diagnosis. Although the term `AI' is commonly used, recent success in its applications to medicine is mainly due to advancements in the sub-field of machine learning, which has been used to automatically classify images and predict medical outcomes. Powerful machine learning techniques have been harnessed to understand nuances in patient data and medical images, aiming for consistent diagnosis and stratification of disease severity. This is the first literature review on the use of AI in DED. We provide a brief introduction to AI, report its current use in DED research and its potential for application in the clinic. Our review found that AI has been employed in a wide range of DED clinical tests and research applications, primarily for interpretation of interferometry, slit-lamp and meibography images. While initial results are promising, much work is still needed on model development, clinical testing and standardisation.

==> Dry Eye AI review/tables/table-data2.tex <==
\begin{landscape}
\begin{table}
    \caption{\label{tab:datatable}Overview of the data applied for the analyses. %Abbreviations: CV = crossvalidation; * = For multivariate analysis model, but the number of samples was not mentioned
    }
    \centering
    \tiny
    \begin{tabular}{lllll} 
    %\begin{tabular}{llp{3cm}p{3cm}l} 
    %\begin{tabular}{p{0.2\textwidth}p{0.2\textwidth}
    %p{0.1\textwidth}p{0.3\textwidth}p{0.2\textwidth}
    %p{0.2\textwidth}p{0.4\textwidth}} 
    \toprule 
         Study & Type of Input Data & Training Dataset & Testing Dataset & Reference Standard  \\
         \midrule
         \textbf{Clinical Investigations}   \\
         Aggarwal S et al. ($2021$)~\cite{aggarwal2021immunecell} & Tabular & $349$ & Nan & Nan (clinical test results, subjective report)  \\
         Deng X ($2021$)~\cite{DENG2021TearMeniscus} & Images & $253$ (images) & $232$ (images) & Senior clinician\\
         Elsawy A et al. ($2021$)~\cite{ELSAWY2021252} & Images & $29172$ (train), $7293$ (val) & $23760$ & Certified cornea specialist  \\
         Khan ZK et al. ($2021$)\cite{Khan2021image} & Images & $90$ & $22$ & Clinician  \\
         Xiao P et al. ($2021$)~\cite{xiao2021Meibo} & Images & $15$ & Nan & $2$ ophthalmologists \\
         Yeh C-H et al. ($2021$)~\cite{yeh2021Meibo} & Images & $398$ (train), $99$ (val) & $209$ & Trained clinician \\
         da Cruz LB et al. ($2020$)\cite{dacruz2020interferometer} & Tabular & $106$ ($10$-fold CV) & Nan & Optometrist  \\
         da Cruz LB et al. ($2020$)~\cite{dacruz2020ripleysk} & Tabular & $106$ ($10$-fold CV) & Nan & Optometrist  \\
         Fu P-I et al. ($2020$)~\cite{Fu2020LLT} & Tabular & $28$ & Nan & Nan (clinical test results, subjective report) \\
         Fujimoto K et al. ($2020$)~\cite{fujimoto2020comparison} & Tabular & $195$ & Nan & Nan (kerato-conjunctival staining for \ac{DED}) \\
         Maruoka S et al. ($2020$)~\cite{Maruoka2020Meibo} & Images & $221$ ($5$-fold CV) & Nan & $3$ eyelid specialists \\
         Prabhu SM et al.($2020$)~\cite{Prabhu2020Meibo} & Images & $600$ & $200$ & Clinical experts \\
         Stegmann H et al. ($2020$)~\cite{Stegmann2020TearMeniscus} & Images & $6658$ (images) ($5$-fold CV) & Nan & Experienced investigator \\ 
         Wei S et al. ($2020$)~\cite{wei2020therapeutic} & Images & $5000$* & $53$ ($3-5$ per patient) & Experienced investigator  \\
         Giannaccare G et al. ($2019$)~\cite{Giannaccare2019SubbasalNerve} & Tabular & Nan & $69$ & Experienced investigator~\cite{Chen2017ACCMed} \\
         Llorens-Quintana et al. ($2020$)~\cite{Llorens-QuintanaClara2019ANAA} & Images & $149$ & Nan & Clinicians \\
         Wang J et al. ($2019$)~\cite{Wang2019Meibo} & Images & $398$ (train) $99$ (val) & $209$ & Experienced clinician \\
         Yabusaki K et al. ($2019$)~\cite{yabusaki2019diagnose} & Tabular & $93$** & $45$** & Skilled ophthalmologist \\
         Yang J et al. ($2019$)~\cite{yang2019meniscus} & Images & $520$ & Nan & ImageJ software  \\
         Szyperski PD ($2018$)~\cite{Szyperski2018fractal} & Tabular & $110$ & Nan & Nan \\
         Hwang H et al. ($2017$)~\cite{hwang2017image} & Frames & $34$ & Nan & Meibomian gland expert \\
         Koprowski R et al. ($2017$)~\cite{Koprowski2017Meibo} & Images & $228$ (images) & Nan & Specialized clinicians \\
         Peteiro-Barral D et al. ($2017$)~\cite{peteiro2017evaluation} & Tabular & $105$ (LOO CV) & Nan & Experts  \\
         Koprowski R et al. ($2016$)~\cite{Koprowski20161Meibo} & Images & $172$ (images) & Nan & Ophthalmology expert \\
         Remeseiro B et al. ($2016$)~\cite{remeseiro2016iDEAS} & Tabular & Nan & $128$ & Optometrists \\
         Remeseiro B et al. ($2016$)~\cite{remeseiro2016CASDES} & Tabular & Sampled from test set & $50$ & $4$ optometrists \\
         Kanellopoulos AJ et al. ($2014$)~\cite{kanellopoulos2014invivo} & Tabular & $140$ & Nan & Ophthalmologist \\
         Ramos L et al. ($2014$)~\cite{ramos2014automatic} & Videos & $18$ & Nan & $2$/$4$ experts  \\
         Ramos L et al. ($2014$)~\cite{Ramos2014CCLRU} & Videos & $12$ & $6$ & $4$ experts  \\
         Remeseiro et al. ($2014$)~\cite{remeseiro2014tearfilm} & Tabular & $511$ ($10$-fold CV) & Nan & Experts \\
         García-Resúa C et al. ($2013$)~\cite{garcia2013new} & Tabular & $105$ ($6$-fold CV) & Nan & Experienced investigator  \\
         Rodriguez R et al. ($2013$)~\cite{Rodriguez2013Redness} & Tabular & $99$ (images) & Nan & $5$ trained investigators \\
         Koh YW et al. ($2012$)~\cite{koh2012detection} & Tabular & $28$*** & $27$*** & Experts  \\
         Yedidya T et al. ($2009$)~\cite{yedidya2009enforcing} & Videos & $22$ & Nan & Clinician  \\
         Yedidya T et al. ($2007$)~\cite{yedidya2007automatic} & Frames & $8$**** & Nan & Optometrist (evaluated $3$ of the $8$ patients)  \\
         Mathers WD et al. ($2004$)~\cite{mathers2004cluster} & Tabular & $513$ ($10$-fold CV) & Nan & Nan (clinical test results)  \\
         
         \hline
         \textbf{Biochemical Investigations} \\
         
         Cartes C et al. ($2019$)~\cite{cartes2019dry} & Tabular & $40$ (noise added) & $40$ (no noise) & Nan (clinical test results, subjective report)  \\
         Jung JH et al. ($2017$)~\cite{jung2017proteomic} & Tabular & $10$ & Nan & Ophthalmologist  \\
         Gonzalez N et al. ($2014$)~\cite{Gonzalez2014Protein} & Tabular & $70$\% of $93$** & $30$\% of $93$** & Nan (clinical tests) \\
         Grus FH et al. ($2005$)~\cite{grus2005seldi} & Tabular & $50$ \% of $159$ & $50$ \% of $159$ & Nan (clinical test results, subjective report)  \\
         Grus FH et al. ($1999$)~\cite{grus1999analysis} & Tabular & $30$ & $30$ & Nan (clinical test results, subjective report)  \\
         Grus FH et al. ($1998$)~\cite{grus1998clustering} & Tabular & $119$ & $\oplus$ & Nan (clinical test results, subjective report)  \\
         
         \hline
         \textbf{Demographical Investigations} \\
         
         Choi HR et al. ($2020$)~\cite{choi2020association} & Tabular & $2272$ & Nan & Nan (subjective report)  \\
         Nam SM et al. ($2020$)~\cite{nam2020explanatory} & Tabular & $80$ \% of $4391$ & $20$ \% of $4391$ & Ophtalmologist   \\
         Kaido M et al. ($2015$)~\cite{Kaido2015computer} & Tabular & $369$ & Nan & Dry eye specialists  \\
         
        \bottomrule
        
        \multicolumn{5}{p{.7\linewidth}}{Abbreviations: Nan = not available; val = validation; CV = crossvalidation; DED = dry eye disease; LOO = leave one out; * = pretraining images; ** = randomly selected samples, process repeated $10$ times; *** = randomly selected samples, process repeated $100$ times; **** = $3 - 5$ sequences of video per patient; $\oplus$ = For multivariate analysis model, but the number of samples was not mentioned}
    \end{tabular}
\end{table}
\end{landscape}

==> Dry Eye AI review/tables/table-studies-biochem_pop.tex <==
\begin{landscape}
\begin{table}
%   \scriptsize
    \tiny
    \caption{\label{tab:biochemicaltable}Overview of the reviewed studies using biochemical investigations.
    }
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.1\textwidth}
    p{0.05\textwidth}p{0.2\textwidth}p{0.1\textwidth}
    p{0.2\textwidth}p{0.4\textwidth}} 
    %\begin{tabular}{p{2.3cm}p{2.7cm}p{1cm}p{3cm}p{2.5cm}p{3cm}p{6.3cm}} 
    \toprule 
         Study & Objective & N & Clinical Tests & Type of Data & Type of Algorithm & Performance Score(s)  \\
         \midrule
         %\textbf{Biochemical Investigations} \\
         
         Cartes C et al. ($2019$)~\cite{cartes2019dry} & Diagnose DED & $40$ & Tear-Lab Osmometer & Tear osmolarity measurements & LR, Naive Bayes, SVM, RF & LR: accuracy = $85$\%\\
         Jung JH et al. ($2017$)~\cite{jung2017proteomic} & Detect protein patterns in DED & $10$ & Pooled tear and lacrimal fluid, analysed with LC-MS, trypsin digestion, RP-LC fractionation & Proteins in tears and lacrimal fluid & "Network model" based on betweenness centrality & Nan\\
         Gonzalez N ($2014$)~\cite{Gonzalez2014Protein} & Diagnose DED & $93$ & Peptide/protein analysis: gel electrophoresis (SDS-PAGE) & Peptides and proteins in tears & Discriminant analysis, PCA, NN & Accuracy = $89.3$\%, CTRL: sensitivity = $0.99$, specificity = $0.96$, MGD: sensitivity = $0.85$, specificity = $0.96$, aqueous-deficient DED: sensitivity = $0.83$, specificity = $0.93$* \\
         Grus FH et al. ($2005$)~\cite{grus2005seldi} & Diagnose DED & $159$ & Schirmer´s test with anesthesia, tears analysed by LC-MS & Proteins in tears & Discriminant analysis, DNN (used sequentially) & AUROC = $0.93$, sensitivity and specificity = ``approx. $90$\% each''\\
         Grus FH et al. ($1999$)~\cite{grus1999analysis} & Diagnose DED & $60$ & Protein analysis: gel electrophoresis (SDS-PAGE) & Proteins in tears  & DNN, discriminant analysis & DNN: accuracy = $89$\%, discriminant analysis: accuracy = $71$\%\\
         Grus FH et al. ($1998$)~\cite{grus1998clustering} & Diagnose DED & $119$ & Protein analysis: gel electrophoresis (SDS-PAGE) & Proteins in tears & Principal component analysis, K-means clustering (used sequentially), discriminant analysis & K-means: accuracy = $71$\% (DED vs CTRL) and $42$\% (DED, diabetes-DED, CTRL), discriminant analysis: accuracy = $72$\% (DED vs CTRL) and $43$\% (DED, diabetes-DED, CTRL) \\
         \bottomrule
         \multicolumn{7}{p{\linewidth}}{Abbreviations: N = number of subjects; DED = dry eye disease; LR = logistic regression; SVM = support vector machine; RF = random forest; AUROC = area under reciever operating characteristic curve; MGD = meibomian gland dysfunction; CTRL = healthy; DNN = deep neural network; Nan = not available; NN = neural network; LC-MS = liquid chromotography mass spectometry; RP-LC = reverse-phase liquid chromatography; SDS-PAGE = sodium dodecyl sulphate-polyacrylamide gel electrophoresis; OSDI = ocular surface disease index; * = metrics are calculated as the average of $10$ repetitions} \\
    \end{tabular}
\end{table}

\begin{table}
%   \scriptsize
    \tiny
    \caption{\label{tab:populationtable}Overview of the reviewed studies using demographical investigations.
    }
    \centering
   \begin{tabular}{p{0.1\textwidth}p{0.1\textwidth}
    p{0.05\textwidth}p{0.2\textwidth}p{0.1\textwidth}
    p{0.2\textwidth}p{0.4\textwidth}}  
    %\begin{tabular}{p{2.3cm}p{2.7cm}p{1cm}p{3cm}p{2.5cm}p{3cm}p{6.3cm}}  % Backup
    \toprule 
         Study & Objective & N & Clinical Tests & Type of Data & Type of Algorithm & Performance Score(s)  \\
         \midrule
         %\textbf{Demographical Investigations} \\
         
         Choi HR et al. ($2020$)~\cite{choi2020association} & Investigate DED and dyslipidemia association & $2272$ & OSDI score, health examination, questionnaire & Population studies, Korea & GLM, LR & Nan\\
         Nam SM et al. ($2020$)~\cite{nam2020explanatory} & Detect risk factors for DED & $4391$ & Health examination, health survey, nutrition survey & National health survey, Korea &  Decision tree, Lasso, LR (used sequentially) & AUROC = $0.70$,  $95$\% CI = $0.61 - 0.78$, specificity = $68$\%, sensitivity = $66$\%\\
         Kaido M et al. ($2015$)~\cite{Kaido2015computer} & Diagnose DED & $369$ & Blink frequency, visual maintenance ratio, questionnaire & Functional VA measurement and questionnaire, Japanese visual display terminal workers & Discriminant analysis & sensitivity = $93.1$\%, specificity = $43.7$\%, precision = $83.8$\%, NPV = $80.8$\%\\
         \bottomrule
         \multicolumn{7}{p{\linewidth}}{Abbreviations: N = number of subjects; DED = dry eye disease; GLM = generalized linear model; AUROC = area under reciever operating characteristic curve; Nan = not available; CI = confidence interval;  LR = logistic regression; OSDI = ocular surface disease index; VA = visual acuity; NPV = negative predictive value} \\
    \end{tabular}
\end{table}
\end{landscape}

==> Dry Eye AI review/tables/table-studies-clinical_part1.tex <==
\begin{landscape}
\begin{table}
%   \scriptsize
    \tiny
    \caption{\label{tab:clinicaltable_1}Overview of the reviewed studies using clinical investigations, part 1 of 2.
    }
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.1\textwidth}
    p{0.05\textwidth}p{0.2\textwidth}p{0.1\textwidth}
    p{0.2\textwidth}p{0.4\textwidth}}  
    \toprule 
         Study & Objective & N & Clinical Tests & Type of Data & Type of Algorithm & Performance Score(s)  \\
         \midrule
         %\textbf{Clinical Investigations} \\
         Aggarwal S et al. ($2021$)~\cite{aggarwal2021immunecell} & DED mechanism, effect of therapy & $199$ & Subjective symptoms, Schirmer´s test with anasthesia, TBUT, vital staining of cornea and conjunctiva, laser IVCM images, subbasal layer of cornea: DC density and morphology & Images of cornea & GLM, MLR & GLM: p-values < $0.05$ for DC density and number of DCs, MLR: p-values < $0.05$ between DC density and CFS, number of DCs and CFS, DC size and CFS, DC density and conjunctival staining, number of DCs and TBUT, corresponding $\beta$-coefficients = $0.20$, $-0.23$, $0.36$, $0.24$ and $-0.18$ \\
         Deng X et al. ($2021$)~\cite{DENG2021TearMeniscus} & Estimate tear meniscus height & $217$ & Oculus Keratograph & Tear meniscus images & CNN (U-net) & Accuracy = $82.5$\%, sensitivity = $0.899$, precision = $0.911$, F1 score = $0.901$ \\
         
         Elsawy A et al. ($2021$)~\cite{ELSAWY2021252} & Diagnose DED & $547$ & AS-OCT & Ocular surface images & Pretrained CNN (VGG19) & AUCROC = $0.99$ (model $1$) and $0.98$ (model $2$), AUCPRC = $0.96$ (model $1$) and $0.94$ (model $2$), F1 score = $0.90$ (model $1$) and $0.86$ (model $2$)* \\
         Khan ZK et al. ($2021$)\cite{Khan2021image} & Detect MGD & $112$ & Meibomian gland 3D IR-images, lower and upper eyelid & Meibomian gland images & GAN & F1 score = $0.825$, P-HD = $4.611$, aggregated JI = $0.664$, r = $0.962$ (clincian1) and $0.968$ (clinician2), p-values < $0.001$, mean difference = $0.96$ (clincian1) and $0.95$ (clincian2) \\
         Xiao P et al.($2021$)~\cite{xiao2021Meibo} & Detect MGD & $15$ (images) & Oculus Keratograph & IR meibography images & Prewitt operator, Graham scan algorithm, fragmentation algorithm and SA (used sequentially) & Gland area: KI = $0.94$, FPR = $6.02$\%, FNR = $6.43$\%. Gland segmentation: KI = $0.87$, FPR = $4.35$\%, FNR = $18.61$\%*  \\
         Yeh C-H et al. ($2021$)~\cite{yeh2021Meibo} & Detect MGD & $706$ (images) & Oculus Keratograph & IR meibography images & Nonparametric instance discrimination, pretrained CNN (ImageNet), hierarchical clustering & : Accuracy: meiboscore grading = $80.9$\%, 2-class classification = $85.2$\%, 3-class classification = $81.3$\%, 4-class classification = $80.8$\%*  \\
         da Cruz LB et al. ($2020$)\cite{dacruz2020interferometer} & Classify tear film patterns & $106$ (images) & Doane interferometer & Tear film lipid layer images & SVM, RF, RT, Naive Bayes, DNN, simple NN & RF: accuracy = $97.54$\%, SD = $0.51$\%, F1 score = $0.97$, KI = $0.96$, AUCROC = $0.99$**  \\
         da Cruz LB et al. ($2020$)~\cite{dacruz2020ripleysk} & Classify tear film patterns & $106$ (images) & Doane interferometer & Tear film lipid layer images & SVM, RF, RT, Naive Bayes, DNN, simple NN  & RF: accuracy = $99.622$\%, SD = $0.843$\%, F1 score = $0.996$, KI = $0.995$, AUCROC = $0.999$*** \\
         Fu P-I et al. ($2020$)~\cite{Fu2020LLT} & Compare $2$ methods & $28$ & Oculus Keratograph & Tear film lipid layer images (with and without preprocessing) & GLM & $\beta$-coefficients = $0.6$, $10$ \\ 
         Fujimoto K et al. ($2020$)~\cite{fujimoto2020comparison} & Compare $2$ methods & $195$ & Pentacam vs AS-OCT  & CCT, TCT, thinnest point of cornea & Multivariable regression & Severe DED: $\beta$-coefficients = $7.029$ (CCT) and $6.958$ (TCT), p-values = $0.002$ (CCT) and $0.049$ (TCT), $95$\% CI = $2.528-11.530$ (CCT) and $0.037-13.879$ (TCT) \\
         Maruoka S et al. ($2020$)~\cite{Maruoka2020Meibo} & Detect MGD & $221$ & IVCM & Meibomian gland images & Combinations of $9$ CNNs & Single CNN: AUROC = $0.966$, sensitivity = $0.942$, specificity = $0.821$, ensemble CNNs: AUROC = $0.981$, sensitivity = $0.921$, specificity = $0.988$ \\
         Prabhu SM et al. ($2020$)~\cite{Prabhu2020Meibo} & Quantify and detect MGD & $400$ (images) & Oculus Keratograph, digital camera & CNN (U-net) & $p$-values > $0.005$ between model output and clinical experts \\
         Stegmann H et al. ($2020$)~\cite{Stegmann2020TearMeniscus} & Detect tear meniscus in images & $10$ & Optical coherence tomography & Tear meniscus images & $2$ CNNs & Meniscus localization: JI = $0.7885$, sensitivity = $0.9999$, meniscus segmentation best CNN: accuracy = $0.9995$, sensitivity = $0.9636$ , specificity = $0.9998$, JI = $0.9324$, F1 score = $0.9644$, support = $0.0071$*, *** \\
         Wei S et al. ($2020$)~\cite{wei2020therapeutic} & DED mechanism, effect of therapy & $53$ & Corneal IVCM with anesthesia & Images of cornea & Pretrained CNN (U-net) & AUROC = $0.96$,  sensitivity = $96$\% \\
         Giannaccare G et al. ($2019$)~\cite{Giannaccare2019SubbasalNerve} & Subbasal nerve plexus characteristics for diagnosing DED & $69$ & IVCM & Images of subbasal nerve plexus & Earlier developed method involving RF and NN~\cite{Chen2017ACCMed, Dabbah2011NerveFiber} & Nan \\
         \bottomrule
         \multicolumn{7}{p{\linewidth}}{Abbreviations: N = number of subjects; DED = dry eye disease; IVCM = in vivo confocal microscopy; DC = dendritic cell; GLM = generalized linear model; MLR = multiple linear regression; CFS = corneal fluorescein score;  AS-OCT = anterior segment optical coherence tomography; CNN = convolutional neural network; AUROC = area under reciever operating characteristic curve; AUPRC = area under precision-recall curve; MGD = meibomian gland dysfunction; GAN = generative adversarial network; P-HD = average Pompeiu-Hausdorff distance; JI = Jaccard index; KI = Kappa index; CTRL = healthy; FPR = false positive rate; FNR = false negative rate; SVM = support vector machine; RF = random forest; RT = random tree; DNN = deep neural network; SD = standard deviation; CCT = central corneal thickness; TCT = thinnest corneal thickness; r = Pearson's correlation coefficient;Nan = not available; NN = neural network; RMSE = root mean squared error; CI = confidence interval;  TBUT = fluorescein tear break-up time; PA = pruning algorithm; SA = skeletonization algorithm; FFA = Flood-fill algorithm; * = standard deviations not included in table; ** = $95$\% confidence intervals not included in table; *** = metrics are calculated as the average of $5$ repetitions;**** = metrics are calculated as the average of $10$ repetitions; ***** = metrics are calculated as the average from $10$-fold crossvalidation; $\ominus$ = metrics are calculated as the average from $6$-fold crossvalidation $\oplus$ = metrics are calculated as the average of $100$ models)} \\
    \end{tabular}
\end{table}
\end{landscape}

==> Dry Eye AI review/tables/table-studies-clinical_part2.tex <==
\begin{landscape}
\begin{table}
%   \scriptsize
    \tiny
    \caption{\label{tab:clinicaltable_2}Overview of the reviewed studies using clinical investigations, part 2 of 2.
    }
    \centering
    \begin{tabular}{p{0.1\textwidth}p{0.1\textwidth}
    p{0.05\textwidth}p{0.2\textwidth}p{0.1\textwidth}
    p{0.2\textwidth}p{0.4\textwidth}} 
    \toprule 
         Study & Objective & N & Clinical Tests & Type of Data & Type of Algorithm & Performance Score(s)  \\
         \midrule
         %\textbf{Clinical Investigations} \\
        Llorens-Quintana C et al. ($2019$)~\cite{Llorens-QuintanaClara2019ANAA} & Evaluate meibomian gland atrophy & $149$ & Oculus Keratograph & Meibography images & Sobel operator, polynomial function, fragmentation algorithm, Otsu's method (used sequentially) & $p$-values < $0.05$ between automatic method and clinicians \\
        Wang J et al. ($2019$)~\cite{Wang2019Meibo} & Evaluate meibomian gland atrophy & $706$ (images) & Oculus Keratograph & Meibography images & $4$ CNNs & Meiboscore grading: accuracy = $95.6$\%, eyelid detection: accuracy = $97.6$\%, JI = $0.955$, atrophy detection: accuracy = $95.4$\%, JI = $0.667$, RMSE = $0.067$ (average across $4$ meiboscores) \\
         Yabusaki K ($2019$)~\cite{yabusaki2019diagnose} & Diagnose DED & $138$ (images) & Tear interferometer & Tear film lipid layer images & SVM & KI = $0.820$, CTRL: F1 score = $0.845$, SD = $0.067$, aqueous-deficient DED: F1 score = $0.981$, SD = $0.023$, evaporative DED: F1 score = $0.815$, SD = $0.095$**** \\
         Yang J et al. ($2019$)~\cite{yang2019meniscus} & Estimate tear meniscus height for DED & $69$ & Slit-lamp images with fluorescence staining & Ocular surface images & Connected component labelling & Mean: p-value < $0.01$ (x$16$ and x$40$ magnification), r = $0.626$ (x$16$) and  $0.711$ (x$40$), max: p-value < $0.001$ (x$16$ and x$40$), r = $0.645$ (x$16$) and $0.847$ (x$40$) \\
         Szyperski PD ($2018$)~\cite{Szyperski2018fractal} & Diagnose DED & $110$ & Interferometry & Videos from lateral shearing interferometry & $4$ different fractal dimension estimators, linear regression & Best estimator: AUROC = $0.786$ \\
         Hwang H et al. ($2017$)~\cite{hwang2017image} & Estimate tear film lipid layer thickness & $34$ & Lipiscanner $1.0$, slit-lamp microscope & Tear film lipid layer videos & Flood-fill algorithm, Canny edge detection & p-value < $0.01$ between all MGD groups \\
         Koprowski R et al. ($2017$)~\cite{Koprowski2017Meibo} & Detect MGD & $57$ & Oculus Keratograph & Meibography images & Riesz pyramid (?), Bezier curve (used sequentially) & Accuracy = $99.08$\%, sensitivity = $1$, specificity = $0.98$\\
         Peteiro-Barral D et al. ($2017$)~\cite{peteiro2017evaluation} & Classify tear film patterns & $105$ (images) & Tearscope plus images & Tear film lipid layer images & SVM, Decision tree, Naive Bayes, simple NN, Fisher´s linear discriminant & NN: accuracy = $96$\%, sensitivity = $92$\%, specificity = $97$\%, precision = $92$\%, F1 score = $0.93$, AUCROC = $0.95$ \\ 
         Koprowski et al. ($2016$)~\cite{Koprowski20161Meibo} & Detect MGD & $86$ & Oculus Keratograph & Meibography images & Otsu's method, SA, watershed algorithm (used sequentially) & Sensitivity = $0.993$, specificity = $0.975$ \\
         Remeseiro B et al. ($2016$)~\cite{remeseiro2016iDEAS} & Classify tear film patterns & $128$ (images) & Tearscope-plus images & Tear film lipid layer images & SVM & accuracy = $96.09$\%, precision = $92.00$\%, sensitivity = $89.66$\%, specificity = $97.98$\%, F1 score = $91.23$\%, processing time = $0.07$ s\\
         Remeseiro B et al. ($2016$)~\cite{remeseiro2016CASDES} & Classify tear film patterns & $50$ (images) & Tearscope-plus images & Tear film lipid layer images & SVM & accuracy = $90.89$\%, sensitivity = $83.54$\%, precision = $97.95$\%, specificity = $86.75$\% \\
         Kanellopoulos AJ et al. ($2014$)~\cite{kanellopoulos2014invivo} & Diagnose DED & $70$ & Fourier-domain AS-OCT system: corneal and corneal epithelial thickness maps & Corneal examination & Linear regression (correlation between DED and thickness) & Nan \\
         Ramos L et al. ($2014$)~\cite{ramos2014automatic} & Estimate TBUT & $18$ (videos) & Videos from TBUT (slit-lamp) & TBUT videos & Polynomial function & specificity = $89$\% (parameter b) and $82$\% (parameter e), specificity = $84$\% and $80$\% \\
         Ramos L et al. ($2014$)~\cite{Ramos2014CCLRU} & Estimate TBUT & $18$ (videos) & Videos from TBUT (slit-lamp) & TBUT videos & Polynomial function & accuracy = "more than $90$\%" \\
         Remeseiro et al. ($2014$)~\cite{remeseiro2014tearfilm} & Classify tear film patterns & $511$ (images) & Tearscope-plus images & Tear film lipid layer images & Markov random field, SVM (used sequentially) & accuracy = $97.14$\%, accuracy (noisy data) = $92.61\%$*****\\ 
         García-Resúa C et al. ($2013$)~\cite{garcia2013new} & Classify tear film patterns & $105$ & Tearscope-plus images & Tear film lipid layer images & K-nearest neighbors & Cram{\'e}r's V = $0.9$, r = $0.94$, p-value < $0.001$, accuracy = $86.2$\% $\ominus$\\
         Rodriquez JD ($2013$)~\cite{Rodriguez2013Redness} & Evaluate ocular redness & $26$ & Slit-lamp, digital camera & Images of conjunctiva & Sobel operator, MLR (used sequentially) & Accuracy = $100$\%, r = $0.76$, concordance correlation = $0.76$ (compared to $5$ investigators)*\\
         Koh YW et al. ($2012$)~\cite{koh2012detection} & Detect MGD & $55$ & Slit-lamp biomicroscope, upper eye lid & IR meibography images & PA, SA, FFA, SVM (used sequentially) & specificity = $96.1$\%, SD = $0.4$\%, sensitivity = $97.9$\%, SD = $0.6$\% $\oplus$\\
         Yedidya T et al. ($2009$)~\cite{yedidya2009enforcing} & Estimate TBUT & $22$ (videos) & Video from TBUT & TBUT videos & Markov random field  & average difference in TBUT = $2.34$s \\
         Yedidya T et al. ($2007$)~\cite{yedidya2007automatic} & Detect dry areas & $8$ (videos) & Video from TBUT & TBUT videos & Levenberg-Marquardt & accuracy = $91$\% ($84-96$\%), SD = $4$\%\\
         Mathers WD et al. ($2004$)~\cite{mathers2004cluster} & Investigate DED & $513$ & Schirmer´s test, meibomian gland drop-out, lipid viscosity and volume, tear evaporation & Clinical test results & Hierarchical clustering, decision tree & Nan\\
         \bottomrule
         \multicolumn{7}{p{\linewidth}}{Abbreviations: N = number of subjects; DED = dry eye disease; IVCM = in vivo confocal microscopy; DC = dendritic cell; GLM = generalized linear model; MLR = multiple linear regression; CFS = corneal fluorescein score;  AS-OCT = anterior segment optical coherence tomography; CNN = convolutional neural network; AUROC = area under reciever operating characteristic curve; AUPRC = area under precision-recall curve; MGD = meibomian gland dysfunction; GAN = generative adversarial network; P-HD = average Pompeiu-Hausdorff distance; JI = Jaccard index; KI = Kappa index; CTRL = healthy; FPR = false positive rate; FNR = false negative rate; SVM = support vector machine; RF = random forest; RT = random tree; DNN = deep neural network; SD = standard deviation; CCT = central corneal thickness; TCT = thinnest corneal thickness; r = Pearson's correlation coefficient;Nan = not available; NN = neural network; RMSE = root mean squared error; CI = confidence interval;  TBUT = fluorescein tear break-up time; PA = pruning algorithm; SA = skeletonization algorithm; FFA = Flood-fill algorithm; * = standard deviations not included in table; ** = $95$\% confidence intervals not included in table; *** = metrics are calculated as the average of $5$ repetitions;**** = metrics are calculated as the average of $10$ repetitions; ***** = metrics are calculated as the average from $10$-fold crossvalidation; $\ominus$ = metrics are calculated as the average from $6$-fold crossvalidation $\oplus$ = metrics are calculated as the average of $100$ models)} \\
    \end{tabular}
\end{table}
\end{landscape}
